Stepwise Self-Consistent Mathematical Reasoning with Large Language Models

Using Large Language Models for complex mathematical reasoning is difficult, primarily due to the complexity of multi-step reasoning. The main challenges of this process include (1) selecting critical intermediate results to advance the procedure, and (2) limited exploration of potential solutions. To address these issues, we introduce a novel algorithm, namely Stepwise Self-Consistent Chain-of-Thought (SSC-CoT). SSC-CoT employs a strategy of selecting intermediate steps based on the intersection of various reasoning chains. Additionally, SSC-CoT enables the model to discover critical intermediate steps by querying a knowledge graph comprising relevant domain knowledge. To validate SSC-CoT, we present a new dataset, TriMaster100, tailored for complex trigonometry problems. This dataset contains 100 questions, with each solution broken down into scored intermediate steps, facilitating a comprehensive evaluation of the mathematical reasoning process. On TriMaster100, SSC-CoT triples the effectiveness of the state-of-the-art methods. Furthermore, we benchmark SSC-CoT on the widely recognized complex mathematical question dataset, MATH level 5, and it surpasses the second-best method by 7.2% in accuracy. Code and the TriMaster100 dataset can be found at: https://github.com/zhao-zilong/ssc-cot.

==> text.tex <==


\section{Algorithm Process Comparison}
\label{appendix:comparison}
\begin{table}
    \centering
    \resizebox{\linewidth}{!} {
    
    \begin{tabular}{{c}}
    \toprule
    $Q$:  What is the smallest integer value of $c$ such that the function $\f(x)=\frac{2x^2+x+5}/{x^2+4x+c}$ has a domain of all real numbers? \\
    \midrule \midrule 
        \textbf{Reasoning from SSC-CoT} \\ 
        ------------------------------------------- \\
        \textbf{Round 1 - Given}: $Q$ \\
        $\mathbf{S}_v$: {$x^2+4x+c = 0$}  \\

        \textbf{Round 2 - Given}: $Q$, $\mathbf{S}_v$\\
        $\mathbf{S}_v$: {$16-4c < 0$}   \\

        \textbf{Round 3 - Given}: $Q$, $\mathbf{S}_v$\\
        $\mathbf{S}_v$:  {$c > 4$}  \\

        \textbf{Result}: $c = 5$ \\
    \midrule \midrule 
    

\textbf{Reasoning from ToT} \\ 
------------------------------------------- \\

    \textbf{Step 1}: We got a conclusion that$ x^2+4x+c$should not equal 0.\\
    \textbf{Step 2}: We further got a conclusion that \textcolor{red}{$b^2-4ac>0$}\\
    \textbf{Step 3}: After putting the values of a and b into $b^2-4ac$ respectively, we get \textcolor{red}{$16-4c > 0 $}\\
    \textbf{Step 4}: Finally, we get  a conclusion ：\textcolor{red}{$c < 4$}\\
    \textbf{Step 5}: So, the answer is \textcolor{red}{$c = 4$}\\
    \bottomrule
    \end{tabular}
    }

  \end{table}%
  
SSC-CoT (Top)and ToT(Below) for addressing algebraic problem. Our SSC-CoT solves this problem correctly based on $\mathbf{S}_v$ highlighted in colors, while ToT makes a factual mistake (in red) and cannot arrive at the correct answer.
